Keeping LLMs Aligned After Fine-tuning: The Crucial Role of Prompt Templates

Public LLMs such as the Llama 2-Chat underwent alignment training and were considered safe. Recently Qi et al. [2024] reported that even benign fine-tuning on seemingly safe datasets can give rise to unsafe behaviors in the models. The current paper is about methods and best practices to mitigate such loss of alignment. We focus on the setting where a public model is fine-tuned before serving users for specific usage, where the model should improve on the downstream task while maintaining alignment. Through extensive experiments on several chat models (Meta's Llama 2-Chat, Mistral AI's Mistral 7B Instruct v0.2, and OpenAI's GPT-3.5 Turbo), this paper uncovers that the prompt templates used during fine-tuning and inference play a crucial role in preserving safety alignment, and proposes the ``Pure Tuning, Safe Testing'' (PTST) strategy -- fine-tune models without a safety prompt, but include it at test time. This seemingly counterintuitive strategy incorporates an intended distribution shift to encourage alignment preservation. Fine-tuning experiments on GSM8K, ChatDoctor, and OpenOrca show that PTST significantly reduces the rise of unsafe behaviors.

==> gpt_gsm8k_other_templates.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{figs/templates-gpt.pdf}
    \caption{The ASR on \ourharmful and the helpfulness for GPT-3.5 Turbo fine-tuned on GSM8K with different training and test templates. The conclusions are similar to those presented in \Cref{fig:llama-other-templates}: fine-tuning with \chatllamasys and inference with another safety prompt still leads to noticeable safety degradation. By contrast, our PTST strategy effectively maintains the safety.}
    \label{fig:gpt-other-templates}

    \vspace{-0.1in}
\end{figure}

==> llama7bchat_gsm8k_other_templates.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{figs/templates.pdf}
    \caption{The ASR on \ourharmful and the helpfulness for Llama 2-7B-Chat fine-tuned on GSM8K with different training and test templates. The results are grouped by the test template, and \texttt{X} denotes template \texttt{chat:X}. Fine-tuning with \chatllamasys and inference with another safety prompt still leads to noticeable safety degradation. By contrast, PTST strategy preserves the safety.}
    \label{fig:llama-other-templates}
\end{figure}

==> mistral_chatdoctor_tables.tex <==
\begin{table*}[t]
\centering
\small
\begin{subtable}{0.28\textwidth}
\centering
    \begin{tabular}{l|c|c|c}
    \diagbox[width=4em]{train}{test} & \shortpurechat & \shortchatalpacasys & \shortchatllamasys \\
    \hhline
    No FT    &  \hlcellc ? & \hlcellc ? & \hlcellc ? \\
    \hhline
    \shortpurechat & \hlcella ?   & 0.846 & \hlcellb 0.846 \\
    \hline
    \shortchatalpacasys & 0.843 & \hlcella 0.845 & \hlcellb 0.844 \\
    \hline
    \shortchatllamasys & 0.845 & 0.846 & \hlcella 0.846 
\end{tabular}
    \subcaption{Helpfulness}
    \label{tab:chatdoctor-helpfulness-mistral}
\end{subtable}%
\begin{subtable}{0.36\textwidth}
\centering
    \begin{tabular}{l|c|c|c}
    \diagbox[width=4em]{train}{test} & \shortpurechat & \shortchatalpacasys & \shortchatllamasys \\
    \hhline
    No FT     & \hlcellc & \hlcellc & \hlcellc \\
    \hhline
    \shortpurechat & \hlcella $1.15_{0.74}$ & $0.12_{0.11}$ & \hlcellb $0.04_{0.09}$\\
    \hline
    \shortchatalpacasys & $0.00_{0.00}$ & \hlcella $1.15_{0.50}$ & \hlcellb $0.00_{0.00}$\\
    \hline
    \shortchatllamasys & $0.04_{0.09}$ & $0.04_{0.09}$  & \hlcella $1.71_{0.69}$
\end{tabular}
    \subcaption{AdvBench}
    \label{tab:chatdoctor-advbench-mistral}
\end{subtable}%
\begin{subtable}{0.36\textwidth} 
\centering
    \begin{tabular}{l|c|c|c}
    \diagbox[width=4em]{train}{test} & \shortpurechat & \shortchatalpacasys & \shortchatllamasys \\
    \hhline
    No FT     & \hlcellc & \hlcellc & \hlcellc\\
    \hhline
    \shortpurechat & \hlcella ${3.05}_{3.02}$ & ${3.80}_{4.20}$ & \hlcellb ${1.50}_{1.43}$  \\
    \hline
    \shortchatalpacasys & ${1.65}_{2.06}$ & \hlcella ${3.05}_{2.71}$ & \hlcellb ${0.70}_{1.23}$  \\
    \hline
    \shortchatllamasys & ${1.75}_{2.41}$ & ${1.60}_{1.88}$ & \hlcella ${3.75}_{3.10}$ 
\end{tabular}
    \subcaption{\ourharmful}
\label{tab:chatdoctor-ourharmful-mistral}
\end{subtable}
\caption{Helpfulness and safety for Llama-2-7B-chat fine-tuned on Chatdoctor. We use temperature $\tau=0.7$ and top p $p=1.0$ for decoding. We report the helpfulness/harmfulness scores averaged over $5$ random seeds for decoding, with the standard deviation in the subscript. We omit the standard deviations for the helpfulness scores as they are less than $5\times 10^{-5}$ for all configurations.}
\end{table*}

